BAR: A Backward Reasoning based Agent for Complex Minecraft Tasks

Large language model (LLM) based agents have shown great potential in following human instructions and automatically completing various tasks. To complete a task, the agent needs to decompose it into easily executed steps by planning. Existing studies mainly conduct the planning by inferring what steps should be executed next starting from the agent's initial state. However, this forward reasoning paradigm doesn't work well for complex tasks. We propose to study this issue in Minecraft, a virtual environment that simulates complex tasks based on real-world scenarios. We believe that the failure of forward reasoning is caused by the big perception gap between the agent's initial state and task goal. To this end, we leverage backward reasoning and make the planning starting from the terminal state, which can directly achieve the task goal in one step. Specifically, we design a BAckward Reasoning based agent (BAR). It is equipped with a recursive goal decomposition module, a state consistency maintaining module and a stage memory module to make robust, consistent, and efficient planning starting from the terminal state. Experimental results demonstrate the superiority of BAR over existing methods and the effectiveness of proposed modules.

==> Sections/intro_old.tex <==
% WWW specific
% Every submission must clearly state how the work is relevant to the Web and to the track in the first page.
% This track is a forum to gather researchers interested in knowledge graphs and other forms of structured data models with machine-interpretable semantics that are being widely adopted for many advanced applications on the Web.
% --- Data modeling to support human-machine intelligence, including, but not limited to LLMs agents, intelligent system behavior, explanations, and user-friendly interactions
% --- Methods, algorithms and applications for the development of semantic models, knowledge graphs and other forms of structured data models with machine-interpretable semantics

\section{Introduction}

% LLM based agent is useful, but suffers from executing complex tasks. So automatically planning is important. 
Large language model~(LLM) based agents, while powerful to support human-machine intelligence, suffer from carrying out complex tasks. Automatic task planning thus has huge potential, as it would enable agents to decompose complex tasks into easily executed steps with good interpretability for machines that can be utilized by many advanced web applications~\cite{zhouwebarena, deng2024mind2web, gurreal}. 

% relared work: current studies mainly focus on forward reasoning paradigm for planning, ignore another type of powerful paradigm: backward reasoning. 
To conduct accurate task planning, a model needs to generate machine-executable steps and organize them into proper sequence. Such steps sequence is called plan. Current studies mainly focus on forward reasoning based methods to generate plans for complex tasks~\cite{huang2022language, huang2024understanding, koh2024tree, yu2024flow, chen-etal-2024-tree}. However, they overlook the potential of backward reasoning, another powerful reasoning paradigm in addition to forward reasoning~\cite{yu2023natural}. We argue that backward reasoning deserves more investigation as it can significantly improve the planning abilities of LLM based agents. To fully explore the potential of backward reasoning, we conduct extensive investigations in a simulation environment called ``Minecraft'', which has the advantages of high degree of freedom, rich tasks and scenarios, and strong controllability. Moreover, Minecraft is an ideal environment because LLM based agents have learned preliminary planning skills through tutorials and community forums on the web during pre-train process. 

% What's the substantial difference between forward and backward reasoning, and how can backward reasoning advance the forward reasoning for planning. (why backward reasoning better ?)
To decompose a complex task into a correct plan, the most critical point is how to achieve the task goal by organizing a sequence of proper steps through planning. 
Here we take a classic task in Minecraft —— ``Obtain 1 \textimage{Icons/diamond_pickaxe.png}~(diamond pickaxe)'' to demonstrate the essential advantage of backward reasoning over forward reasoning for planning. 
As shown in the upper part of Figure~\ref{fig:forward_backward}, when conducting planning by forward reasoning, the agent sequentially infers the steps to be executed starting from the initial state. In the initial state, the agent's inventory is empty, so the first step should be ``Mine \textimage{Icons/oak_log.png}~(log)'' as \textimage{Icons/oak_log.png} is the raw material for most items in Minecraft. After that, there are several items can be chosen to craft for the next step. As more steps being determined, the difficulty of planning gradually increases. The situation becomes extremely complex after the step ``Craft \textimage{Icons/stick.png}~(stick)'', as there are a considerable number of steps can be executed next. 
Planning can be seen as the process of finding a suitable path from the initial state to the terminal state~(where 
the task goal has been achieved)~\cite{poole2010artificial}. By forward reasoning, due to the huge gap between the initial state and the terminal state, it is difficult to infer correct steps from a large number of candidates that are semantically far from the task goal. Moreover, it is hard to infer the required quantity of items for each step, as the items' quantity needs to be calculated based on the entire plan. As a result, forward reasoning faces significant challenges for complex tasks planning. 

However, under the backward reasoning paradigm, the situation becomes much easier. 
As shown in the lower part of Figure~\ref{fig:forward_backward}, when conducting planning by backward reasoning, the agent infers the steps to be executed starting from the terminal state. In the terminal state, the task goal has been achieved and the agent has already obtained 1 \textimage{Icons/diamond_pickaxe.png}~(diamond pickaxe). To achieve this goal, the last step should be ``Craft 1 \textimage{Icons/diamond_pickaxe.png}'' because after executing this step the agent can obtain 1 \textimage{Icons/diamond_pickaxe.png}. Furthermore, to successfully execute the step ``Craft 1 \textimage{Icons/diamond_pickaxe.png}'', the agent needs to prepare the materials for it. So the second to last step should be ``Mine 3 \textimage{Icons/diamond.png}~(diamond)'' as \textimage{Icons/diamond.png} is the key material for crafting \textimage{Icons/diamond_pickaxe.png}. Similarly, the agent can continue to infer the third to last step to support the execution of step ``Mine 3 \textimage{Icons/diamond.png}'', repeating until the entire plan is generated. 
As a consequence, backward reasoning is not hindered by the huge gap between the initial and the terminal states, having the potential for promoting more accurate planning. 

\begin{figure*}[t]
    \centering    
    \includegraphics[width=.95\textwidth]{Pictures/forward_backward_reasoning.png}
    \caption{A toy example showing the essential advantage of backward reasoning over forward reasoning for complex task planning. In Minecraft, most tasks are started by ``Mine log'', and the example in the figure is no exception.}
    \label{fig:forward_backward}
\end{figure*}

\begin{figure*}[t]
    \centering    
    \includegraphics[width=.95\textwidth]{Pictures/defect_of_backward_reasoning.png}
    \caption{The wrong step inferred by backward reasoning due to the lack of the perspective of the states during planning. In Minecraft, the stone can only be obtained below the ground, so it is necessary to reach below the ground first and then mine the stone.}
    \label{fig:defect_of_backward}
\end{figure*}

Although backward reasoning has shown huge potential for more accurate planning, it is not yet a perfect solution. 
By backward reasoning, the agent only considers the goals to be achieved for each step, ignoring its located states before achieving these goals. 
As shown in Figure~\ref{fig:defect_of_backward}, the agent incorrectly infers the step ``Mine \textimage{Icons/cobblestone.png}~(stone)'' immediately after ``Craft 1 \textimage{Icons/wooden_pickaxe.png}~(wooden pickaxe)''. In the end, this step cannot be executed successfully because \textimage{Icons/cobblestone.png} can only be obtained below ground but the agent was still above ground before executing the step ``Mine \textimage{Icons/cobblestone.png}''. Therefore, by backward reasoning, the planning ability of the agent is strongly hindered by the limited perspective of the states in the entire plan. And the inconsistency of states between different steps can lead to generating wrong plans. 

% Why propose such a backward reasoning framework
To address the above shortcomings, we conduct in-depth exploration of forward \& backward reasoning based planning. 
We find that through elaborate design, backward reasoning can promote effective planning, while forward reasoning can compensate for the defect of backward reasoning in lacking the perspective of the states during the planning. Inspired by dynamic programming algorithm~\cite{bellman1954theory}, we propose a re\underline{C}ursive p\underline{L}anning fram\underline{E}work based on b\underline{A}ckward \underline{R}easoning~(\model), which can support accurate planning of complex tasks through three well-designed modules. 

% Experimental setting
We choose the simulation environment ``Minecraft''~\cite{guss2019minerl} to examine the effectiveness of our framework. Minecraft provides a wide range of tasks for agents to conduct planning and execution~\cite{lifshitz2024steve}. To compare the planning ability of our framework with other methods, we select a series of tasks from the build-in technology tree in Minecraft. We first evaluate the accuracy of plans generated by different methods from the textual perspective. We annotate a standard dataset and compute the overlap between the generated plans and the ground truth for evaluation. In addition, we execute the generated plans in the simulation environment to evaluate the execution success rate of generated plans. 

% Experimental results briefly
Experimental results show that our proposed framework outperforms other methods for complex tasks planning by a large margin. Current studies fail to generate accurate plans due to the inherent defects of forward reasoning, especially for plans with long steps. In contrast, our framework is not affected by the steps length of plans and performs robustly in all evaluated tasks. Moreover, after introducing the interaction with the environment, our framework can further unleash its reasoning potential and show powerful planning ability for complex tasks. We hope our exploration and discoveries can promote the development of more efficient agents to support human-machine intelligence. 

% Contributions
In conclusion, our contributions can be three-fold:
\begin{itemize}
    \item We call attention to the backward reasoning based planning, which represents another powerful reasoning paradigm for complex tasks planning except forward reasoning. 
    \item We design a new planning framework based on backward reasoning, equipping it with powerful planning ability and the potential to enhance performance through the interacting with the environment. 
    \item Experimental results demonstrate the superiority of our framework and reveal the advantages of backward reasoning over forward reasoning for complex tasks planning. 
\end{itemize}




==> Tables/dynamic_planning.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[th]
\caption{Results of dynamic task planning experiments. Best results are highlighted in {\color[HTML]{009901} \textbf{bold}}, and the second best results are highlighted with {\ul underline}. ``SR'' refers to the average Success Rate and ``Time'' refers to the average time taken to run the plan.}
\scalebox{.85}{
\begin{tabular}{ll|cc|cc|cc}
\hline
\multicolumn{2}{c|}{}                         & \multicolumn{2}{c|}{diamond}                                                  & \multicolumn{2}{c|}{redstone}                                                 & \multicolumn{2}{c}{gold}                                                      \\ \cline{3-8} 
\multicolumn{2}{c|}{\multirow{-2}{*}{Method}} & SR                                    & Time                                  & SR                                    & Time                                  & SR                                    & Time                                  \\ \hline
\multicolumn{2}{l|}{React}                    & 14.29                                 & {\ul 8m9s}                            & 14.29                                 & 7m57s                                 & 21.43                                 & 8m23s                                 \\
\multicolumn{2}{l|}{Jarvis-1}                 & 10.00                                 & {\color[HTML]{009901} \textbf{7m28s}} & 30.00                                 & {\ul 7m28s}                           & 11.43                                 & 8m7s                                  \\ \specialrule{0em}{1pt}{1pt} \hline
\multicolumn{2}{l|}{Ours}                     &                                       &                                       &                                       &                                       &                                       &                                       \\
\multicolumn{2}{l|}{\quad - static}                   & 31.43                                 & 8m21s                                 & 35.71                                 & 7m53s                                 & 30.00                                 & 7m55s                                 \\
\multicolumn{2}{l|}{\quad - static + React}           & {\ul 40.00} & 9m3s                                  & {\ul 42.86}                           & 8m15s                                 & {\ul 38.57}                           & {\ul 7m44s}                           \\
\multicolumn{2}{l|}{\quad - dynamic}                  & {\color[HTML]{009901} \textbf{41.43}} & 9m9s                                  & {\color[HTML]{009901} \textbf{44.29}} & {\color[HTML]{009901} \textbf{6m55s}} & {\color[HTML]{009901} \textbf{41.43}} & {\color[HTML]{009901} \textbf{7m39s}} \\ \specialrule{0em}{1pt}{1pt} \hline
\end{tabular}
}
\label{tab:dynamic}
\end{table}

==> Tables/dynamic_planning_textual_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[!th]
\caption{Results of the dynamic planning experiments by textual metrics. Best results are highlighted in {\color[HTML]{009901} \textbf{bold}}. For the adopted metrics, ``Acc'' refers to Accuracy, ``F1'' refers to F1-Score, and ``ED'' refers to Edit Distance.}
% \vspace{-7pt}
\scalebox{0.8}{
\begin{tabular}{ll|ccc|ccc|ccc|ccc|ccc|ccc}
\hline
\multicolumn{2}{c|}{}                                & \multicolumn{3}{c|}{{\color[HTML]{262626} \textbf{wood}}}                                                            & \multicolumn{3}{c|}{{\color[HTML]{262626} \textbf{stone}}}                                                           & \multicolumn{3}{c|}{{\color[HTML]{262626} \textbf{iron}}}                                                            & \multicolumn{3}{c|}{{\color[HTML]{262626} \textbf{diamond}}}                                                         & \multicolumn{3}{c|}{{\color[HTML]{262626} \textbf{redstone}}}                                                        & \multicolumn{3}{c}{{\color[HTML]{262626} \textbf{gold}}}                                                             \\ \cline{3-20} 
\multicolumn{2}{c|}{\multirow{-2}{*}{Method}}        
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$            \\ \hline
\multicolumn{2}{l|}{{\color[HTML]{262626} React}}   & 64.52                                 & 66.84                                 & 1.35                                 & 70.33                                 & 72.53                                 & 2.18                                 & 89.17                                 & 89.17                                 & 1.43                                 & {\color[HTML]{262626} 71.17}          & {\color[HTML]{262626} 74.77}          & {\color[HTML]{262626} 4.57}          & 57.01                                 & 57.49                                 & 7.00                                 & 57.63                                 & 79.75                                 & 4.43                                 \\
\multicolumn{2}{l|}{{\color[HTML]{262626} Jarvis-1}} & 61.29                                 & 60.64                                 & 1.65                                 & 75.82                                 & 75.00                                 & 2.09                                 & 73.61                                 & 76.56                                 & 3.38                                 & {\color[HTML]{262626} 81.98}          & {\color[HTML]{262626} 81.98}          & {\color[HTML]{262626} 2.86}          & 70.09                                 & 71.70                                 & 5.00                                 & 52.54                                 & 74.09                                 & 5.71                                 \\ \hline
\multicolumn{2}{l|}{Ours}                            & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                  & \multicolumn{1}{l|}{}                & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                  & \multicolumn{1}{l|}{}                & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                  & \multicolumn{1}{l|}{}                & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                  & \multicolumn{1}{l|}{}                & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                  & \multicolumn{1}{l|}{}                & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                  & \multicolumn{1}{l}{}                 \\
\multicolumn{2}{l|}{{\color[HTML]{262626} \quad - static}}   & {\color[HTML]{262626} 83.87}          & {\color[HTML]{262626} 83.57}          & {\color[HTML]{262626} 0.70}          & {\color[HTML]{262626} 87.91}          & {\color[HTML]{262626} 87.91}          & {\color[HTML]{262626} 1.00}          & {\color[HTML]{262626} 82.67}          & {\color[HTML]{262626} 85.02}          & {\color[HTML]{262626} 2.19}          & {\color[HTML]{262626} 87.39}          & {\color[HTML]{262626} 88.23}          & {\color[HTML]{262626} 1.86}          & {\color[HTML]{262626} 80.53}          & {\color[HTML]{262626} 82.22}          & {\color[HTML]{262626} 2.86}          & 85.59                                 & 87.34                                 & 2.14                                 \\
\multicolumn{2}{l|}{\quad - dynamic}                         & {\color[HTML]{009901} \textbf{89.47}} & {\color[HTML]{009901} \textbf{89.47}} & {\color[HTML]{009901} \textbf{0.43}} & {\color[HTML]{009901} \textbf{92.31}} & {\color[HTML]{009901} \textbf{92.31}} & {\color[HTML]{009901} \textbf{0.64}} & {\color[HTML]{009901} \textbf{96.58}} & {\color[HTML]{009901} \textbf{96.92}} & {\color[HTML]{009901} \textbf{0.45}} & {\color[HTML]{009901} \textbf{88.29}} & {\color[HTML]{009901} \textbf{89.23}} & {\color[HTML]{009901} \textbf{1.71}} & {\color[HTML]{009901} \textbf{86.73}} & {\color[HTML]{009901} \textbf{86.73}} & {\color[HTML]{009901} \textbf{2.14}} & {\color[HTML]{009901} \textbf{86.44}} & {\color[HTML]{009901} \textbf{94.93}} & {\color[HTML]{009901} \textbf{0.86}} \\ \hline
\end{tabular}
}
\label{tab:dynamic_textual}
% \vspace{-3pt}
\end{table*}

==> Tables/static_planning_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\caption{Results of the static planning experiments. Best results are highlighted in {\color[HTML]{009901} \textbf{bold}}, and the second best results are highlighted with {\ul underline}. For the adopted metrics, ``Acc'' refers to Accuracy, ``F1'' refers to F1-Score, and ``ED'' refers to Edit Distance. Larger Accuracy and F1-Score and smaller Edit Distance represent better performance.}
% \vspace{-5pt}
\scalebox{0.8}{
\begin{tabular}{ll|ccc|ccc|ccc|ccc|ccc|ccc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{Method}} & \multicolumn{3}{c|}{\textbf{wood}}                                  & \multicolumn{3}{c|}{\textbf{stone}}                                & \multicolumn{3}{c|}{\textbf{iron}}                                  & \multicolumn{3}{c|}{\textbf{diamond}}                               & \multicolumn{3}{c|}{\textbf{redstone}}                              & \multicolumn{3}{c}{\textbf{gold}}                                  \\ \cline{3-20} 
\multicolumn{2}{c|}{} 
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$
& Acc $\uparrow$  & F1 $\uparrow$  & ED $\downarrow$                   \\ \hline
\multicolumn{2}{l|}{Chain-of-thought}             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{2}{l|}{\quad - Llama-3-8B}              & 47.31                & 46.89                & 2.87                  & 68.97                & 68.13                & 2.91                  & 74.73                & 74.95                & 3.29                  & 55.21                & 51.47                & 8.29                  & 43.69                & 48.45                & 8.57                  & 41.28                & 52.75                & 9.00                 \\
\multicolumn{2}{l|}{\quad - GPT4}                    & 56.99                & 57.66                & 1.78                  & 75.82                & 75.00                & 2.09                  & 77.26                & 78.12                & 2.86                  & 68.47                & 71.94                & 4.29                  & 47.66                & 54.88                & 7.29                  & 52.54                & 73.64                & 5.86                 \\ \specialrule{0em}{1pt}{1pt} \hline

\multicolumn{2}{l|}{Reverse Chain}            & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{2}{l|}{\quad - Llama-3-8B}              & 55.91                & 62.24                & 1.83                  & 22.50                & 44.18                & 5.36                  & 53.28                & 65.01                & 4.67                  & 29.47                & 35.62                & 9.57                  & 13.64                & 20.84                & 12.43                 & 23.81                & 21.23                & 12.86                \\
\multicolumn{2}{l|}{\quad - GPT4}                    & 66.67                & 65.92                & 1.43                  & 73.33                & 74.03                & 2.18                  & {\ul 80.87}          & 81.77                & {\ul 2.43}            & {\ul 86.49}          & {\ul 86.49}          & {\ul 2.14}            & {\ul 77.88}          & {\ul 77.88}          & {\ul 3.57}            & 52.17                & 74.56                & 5.43                 \\ \specialrule{0em}{1pt}{1pt} \hline

\multicolumn{2}{l|}{Self-Refine}             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{2}{l|}{\quad - Llama-3-8B}              & 39.78                & 40.47                & 3.09                  & 65.85                & 63.70                & 3.18                  & 69.23                & 69.58                & 4.05                  & 40.62                & 48.40                & 10.29                 & 40.57                & 47.70                & 8.57                  & 37.27                & 48.92                & 9.57                 \\
\multicolumn{2}{l|}{\quad - GPT4}                    & 54.84                & 55.54                & 1.87                  & 75.82                & 75.00                & 2.09                  & 74.01                & 77.80                & 3.10                  & 74.77                & 79.18                & 3.29                  & 56.88                & 66.64                & 5.71                  & 52.54                & 74.09                & 5.71                 \\ \specialrule{0em}{1pt}{1pt} \hline

\multicolumn{2}{l|}{Tree-of-thought}                     & 42.55                & 47.84                & 2.26                  & 46.91                & 43.92                & 4.27                  & 33.96                & 44.46                & 6.81                  & 38.64                & 28.43                & 10.00                 & 20.43                & 22.23                & 12.14                 & 35.71                & 30.95                & 10.14                \\
\multicolumn{2}{l|}{DEPS}                    & 51.06                & 50.46                & 2.04                  & 49.45                & 46.20                & 3.73                  & 61.01                & 50.35                & 5.24                  & 49.55                & 41.32                & 7.86                  & 26.44                & 25.95                & 11.00                 & 48.65                & 39.42                & 8.14                 \\
\multicolumn{2}{l|}{Plan-and-Solve}          & 47.37                & 53.82                & 2.09                  & 45.45                & 58.29                & 3.45                  & 76.17                & 80.29                & 2.71                  & 66.67                & 77.02                & 4.14                  & 42.06                & 50.67                & 8.43                  & 63.00                & 59.93                & 6.43                 \\
\multicolumn{2}{l|}{Openai-o1}                      & 48.42                & 50.26                & 2.04                  & 74.73                & 74.86                & 2.09                  & 77.98                & {\ul 82.34}          & 2.67                  & 63.96                & 79.55                & 3.57                  & 57.52                & 76.44                & 3.86                  & {\ul 75.42}          & {\ul 83.97}          & {\ul 3.14}           \\ \specialrule{0em}{1pt}{1pt} \hline
\multicolumn{2}{l|}{Ours}                    & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{2}{l|}{\quad - Llama-3-8B}              & {\ul 72.04}          & {\ul 72.09}          & {\ul 1.22}            & {\ul 78.02}          & {\ul 78.02}          & {\ul 1.82}            & 74.44                & 76.00                & 3.33                  & 72.97                & 79.67                & 3.29                  & 59.22                & 59.10                & 7.00                  & 60.71                & 66.38                & 5.86                 \\
\multicolumn{2}{l|}{\quad - GPT4}                    & {\color[HTML]{009901} \textbf{83.87}} & {\color[HTML]{009901} \textbf{83.57}} & {\color[HTML]{009901} \textbf{0.70}} & {\color[HTML]{009901} \textbf{87.91}} & {\color[HTML]{009901} \textbf{87.91}} & {\color[HTML]{009901} \textbf{1.00}} & {\color[HTML]{009901} \textbf{82.67}} & {\color[HTML]{009901} \textbf{85.02}} & {\color[HTML]{009901} \textbf{2.19}} & {\color[HTML]{009901} \textbf{87.39}} & {\color[HTML]{009901} \textbf{88.23}} & {\color[HTML]{009901} \textbf{1.86}} & {\color[HTML]{009901} \textbf{80.53}} & {\color[HTML]{009901} \textbf{82.22}} & {\color[HTML]{009901} \textbf{2.86}} & {\color[HTML]{009901} \textbf{85.59}} & {\color[HTML]{009901} \textbf{87.34}} & {\color[HTML]{009901} \textbf{2.14}} \\ \hline
\end{tabular}
}
\label{tab:static}
% \vspace{-5pt}
\end{table*}
